Entropy Trees and Range-Minimum Queries In Optimal Average-Case Space

The range-minimum query (RMQ) problem is a fundamental data structuring task with numerous applications. Despite the fact that succinct solutions with worst-case optimal $2n+o(n)$ bits of space and constant query time are known, it has been unknown whether such a data structure can be made adaptive to the reduced entropy of random inputs (Davoodi et al. 2014). We construct a succinct data structure with the optimal $1.736n+o(n)$ bits of space on average for random RMQ instances, settling this open problem. Our solution relies on a compressed data structure for binary trees that is of independent interest. It can store a (static) binary search tree generated by random insertions in asymptotically optimal expected space and supports many queries in constant time. Using an instance-optimal encoding of subtrees, we furthermore obtain a "hyper-succinct" data structure for binary trees that improves upon the ultra-succinct representation of Jansson, Sadakane and Sung (2012).

==> preamble.tex <==
% !TeX root = entropy-trees
\makeatletter
\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage{slantsc}

\usepackage{babel}
\input{ushyphex.tex} % hyphenation exceptions


\newcommand{\ifarxiv}[2]{\ifthenelse{\equal{\version}{arxiv}}{#1}{#2}}
\newcommand{\ifconf}[2]{\ifthenelse{\equal{\version}{conference}}{#1}{#2}}
\newcommand{\ifdraft}[2]{\ifthenelse{\equal{\draftmode}{true}}{#1}{#2}}

\usepackage{array,multicol}
\usepackage{amsmath,amsfonts,amssymb,mathtools}
\usepackage{mleftright}\mleftright % redefine left and right to not add space around braces
\usepackage{relsize,ifthen,xspace,enumitem,booktabs,adjustbox,needspace,pbox}
\usepackage{graphicx}





\usepackage{wref}
\usepackage[bibtex]{url-doi-arxiv}




%%%%% pseudocode algorithms
\usepackage{clrscode3e}
\def\Foreach{\kw{for each} }
\def\EndFor{\End\li\kw{end for} }
\def\EndIf{\End\li\kw{end if} }
\def\EndWhile{\End\li\kw{end while} }

%\ifconf{
%	\usepackage{float}
%	\floatstyle{plain}
%	%\floatstyle{plaintop}
%	\DeclareCaptionLabelFormat{boxedalgorithm}{%
%	  \kern0.05em{\color[rgb]{0.99,0.78,0.07}\rule{0.73em}{0.73em}}%
%	  \hspace*{0.67em}\bothIfFirst{Algorithm}{~}#2}
%	\newfloat{algorithm}{tbp}{loa}
%	\floatname{algorithm}{Algorithm}
%	\captionsetup[algorithm]{labelformat=boxedalgorithm}
%	\captionsetup[algorithm]{position=above}
%}{
	\usepackage{newfloat}
	\DeclareFloatingEnvironment[%
			name=Algorithm,%
			placement=thb,%
%			chapterlistsgaps=off%
		]{algorithm}
%}


\usepackage{lscape} % sideways figures
%\usepackage{pdflscape} % use this instead to rotate pdf pages.


%Helper macros

\newcommand\plaincenter[1]{%
	\mbox{}\hfill#1\hfill\mbox{}%
}
\newcommand\plaincenterbox[1]{%
	\mbox{}\hfill\mbox{#1}\hfill\mbox{}%
}













\usepackage{tikz}
\usepackage{relsize}
\usetikzlibrary{positioning,arrows.meta}
\usetikzlibrary{backgrounds,calc,trees,hobby}

\pgfdeclarelayer{background}
\pgfsetlayers{background,main}


% Make title and author accessible in document
\AtBeginDocument{%
	\let\mytitle\@title%
}



%\ifconf{}{
%	\setlength\parindent{1.5em}
%	\usepackage{colonequals}
%%	
%	\usepackage[headsepline]{scrlayer-scrpage}
%	\pagestyle{scrheadings}
%	\clearscrheadfoot
%	\AtBeginDocument{%
%		\manualmark%
%		\markleft{\mytitle}%
%		\automark*[section]{}%
%	}
%	\ohead{\pagemark}
%	\ihead{\headmark}
%%	
%	\addtokomafont{caption}{\sffamily\small}
%	\addtokomafont{captionlabel}{\sffamily\textbf}
%	\setcapmargin{2em}
%}
%


\hypersetup{
	final,
	unicode=true, 
	bookmarks=true,
	bookmarksnumbered=true,
	bookmarksdepth=2,
	bookmarksopen=true,
	breaklinks=true,
	hidelinks,
	pdfhighlight={/P}
}



% Theorems etc
%\ifconf{
	\newtheorem{fact}[theorem]{Fact}
%}{
%	\usepackage[amsmath,hyperref,thmmarks]{ntheorem}
%	
%	\theorembodyfont{\slshape}
%	\theoremseparator{:}
%	\newtheoremstyle{proofstyle}%
%	  {\item[\theorem@headerfont\hskip\labelsep ##1\theorem@separator]}%
%	  {\item[\theorem@headerfont\hskip\labelsep ##1 of ##3\theorem@separator]}
%	
%	%KOMA \theoremstyle{break}
%	%KOMA \theorempreskip{2\topsep}
%	\theorempreskip{\topsep} % new version of ntheorem
%	%\setlength\theorempreskipamount{\topsep} % arxiv version of ntheorem
%	
%	\newtheorem{theorem}{Theorem}[section]
%	
%	\theoremstyle{plain}
%	\theorempreskip{\topsep}
%	
%	\newtheorem{proposition}[theorem]{Proposition}
%	\newtheorem{lemma}[theorem]{Lemma}
%	\newtheorem{conjecture}[theorem]{Conjecture}
%	\newtheorem{corollary}[theorem]{Corollary}
%	\newtheorem{definition}[theorem]{Definition}
%	
%	\theoremstyle{plain}
%	\theorembodyfont{\upshape}
%	
%	\newtheorem{property}[theorem]{Property}
%	\newtheorem{fact}[theorem]{Fact}
%	\newtheorem{remark}[theorem]{Remark}
%	
%	%\theoremsymbol{\ensuremath{_\Box}}
%	\theoremsymbol{\raisebox{-.25ex}{$\Box$}}
%	\qedsymbol{\raisebox{-.25ex}{$\Box$}}
%	
%	
%	\theoremstyle{proofstyle}
%	\newtheorem{proof}{Proof}
%}

\newenvironment{thmenumerate}[2][]{%
	\begin{enumerate}[
		label={\makebox[\widthof{(a)}][c]{\textup{(\alph*)}}},
		ref={\ref{#2}\kern.1em--\kern.1em(\alph*)},
		itemsep=0pt,
		#1
	]%
}{%
	\end{enumerate}%
}




% Plots
\newcommand\mathematicaPlotPdf[2][width=.5\linewidth]{%
	\plaincenter{\includegraphics[#1]{pics/#2}}%
}

%
%\pgfplotsset{
%	legend cell align=left,
%	every axis legend/.append style={%
%		fill=backgroundshading!50!white,
%		rounded corners=1pt,
%	},
%	xlabel near ticks,
%	ylabel near ticks,
%}
%\pgfplotsset{
%	every y tick scale label/.style={
%		at={(-.03,1)},yshift=-1ex,anchor=south east,inner sep=0pt
%	}
%}
%
%\newcommand\mathematicaPlotAxis[3]{% #1=filename #2=axisoptions #3=plotcommands
%	\def\tablefile{pics/#1.tab}%
%	\adjustbox{padding=0pt 0ex 0ex 1ex}{%
%	\externalizedpicture{#1}
%	\begin{tikzpicture}[every node/.style={font=\scriptsize}]
%	\begin{axis}
%	[
%		width=.5\linewidth,
%		height=.38\linewidth,
%		grid=major,
%		cycle list name=coloreddiscreteplots,
%		axis background/.style={fill=backgroundshading!50!white},
%		#2
%	]
%		#3
%	\end{axis}
%	\end{tikzpicture}%
%	}
%}
%\makeatletter
%\def\mathematicaPlotAddPlot{% [options] x y label
%	\@ifstar\@mathematicaPlotAddPlot\@@mathematicaPlotAddPlot%
%}
%\newcommand\@@mathematicaPlotAddPlot[4][]{% [options] x y label
%	\addplot+[#1] table[x=#2,y=#3] {\tablefile} ;
%	\ifthenelse{\equal{#4}{}}{}{\addlegendentry{#4}}
%}
%\newcommand\@mathematicaPlotAddPlot[4][]{% [options] x y label
%	\addplot[#1] table[x=#2,y=#3] {\tablefile} ;
%	\ifthenelse{\equal{#4}{}}{}{\addlegendentry{#4}}
%}
%\makeatother
















%    __  __                          
%   |  \/  | __ _  ___ _ __ ___  ___ 
%   | |\/| |/ _` |/ __| '__/ _ \/ __|
%   | |  | | (_| | (__| | | (_) \__ \
%   |_|  |_|\__,_|\___|_|  \___/|___/
%                                    


% Common phrases
\newcommand*\ie{\mbox{i.\hspace{.2ex}e.}}
\newcommand*\eg{\mbox{e.\hspace{.2ex}g.}}
\newcommand*\iid{\mbox{i.\hspace{.2ex}i.\hspace{.2ex}d.}\xspace}
\newcommand*\wrt{\mbox{w.\hspace{.2ex}r.\hspace{.2ex}t.}\xspace}
\newcommand*\aka{\mbox{a.\hspace{.2ex}k.\hspace{.2ex}a.}\xspace}
\newcommand*\withoutlossofgenerality{\mbox{w.\hspace{.23ex}l.\hspace{.2ex}o.\hspace{.17ex}g.}\xspace}
\newcommand*\Withoutlossofgenerality{\mbox{W.\hspace{.23ex}l.\hspace{.2ex}o.\hspace{.17ex}g.}\xspace}
\newcommand*\almostsurely{\mbox{a.\hspace{.2ex}s.}\xspace}
\newcommand*\whp{\mbox{w.\hspace{.2ex}h.\hspace{.2ex}p.}\xspace}


\newcommand\R{\mathbb R}
\newcommand\N{\mathbb N}
\newcommand\Z{\mathbb Z}
\newcommand\Q{\mathbb Q}
\renewcommand\C{\mathbb{C}}
\newcommand\Oh{O}
\def\.{\mskip1mu} 


\DeclareMathOperator\ld{ld}



\newcommand{\surroundedmath}[3]{% #1=mathrel/mathbin/etc #2=spacing #3=symbol
	\mathchoice{%display
		#1{#2{#3}#2}%
	}{%text
		#1{#3}%
	}{%script
		#1{#3}%
	}{%scriptsript
		#1{#3}%
	}%
}
\newcommand\rel[1]{\surroundedmath{\mathrel}{\:}{#1}}
\newcommand\wrel[1]{\surroundedmath{\mathrel}{\;}{#1}}
\newcommand\wwrel[1]{\surroundedmath{\mathrel}{\;\;}{#1}}
\newcommand\bin[1]{\surroundedmath{\mathbin}{\:}{#1}}
\newcommand\wbin[1]{\surroundedmath{\mathbin}{\;}{#1}}
\newcommand\wwbin[1]{\surroundedmath{\mathbin}{\;\;}{#1}}

\newcommand{\eqwithref}[2][c]{%
	\relwithref[#1]{#2}{=}%
}
\newcommand{\relwithref}[3][c]{%
	\mathrel{\underset{\mathclap{\makebox[\widthof{$=$}][#1]{\scriptsize\wref{#2}}}}{#3}}%
}
\newcommand{\relwithtext}[3][c]{%
	\mathrel{\underset{\mathclap{\makebox[\widthof{$=$}][#1]{\scriptsize#2}}}{#3}}%
}

\newcommand\pe{\phantom{{}={}}}
\newcommand\ppe{\phantom{=}}


\newcommand{\ESymbol}{\mathbb{E}}
\newcommand{\V}{\ensuremath{\mathrm{Var}}}
\newcommand{\Cov}{\ensuremath{\mathrm{Cov}}}
\newcommand{\ProbSymbol}{\ensuremath{\mathbb{P}}}
\providecommand{\given}{}
%% mathtools command to declare cool delimiter pairs:
%	\DeclarePairedDelimiterXPP{cmd}[numargs]{pre code}{left_delim}{right_delim}{post code}{body}
\DeclarePairedDelimiterXPP\Prob[1]{\ProbSymbol}[]{}{%
	\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}%
	#1%
}
\DeclarePairedDelimiterXPP\E[1]{\ESymbol}[]{}{%
	\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}%
	#1%
}
\DeclarePairedDelimiterXPP\Eover[2]{\ESymbol_{#1}}[]{}{%
	\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}%
	#2%
}
\providecommand{\Prob}{} % hack for syntax highlighting ...
\providecommand{\E}{} % hack for syntax highlighting ...
\providecommand{\Eover}{} % hack for syntax highlighting ...




% Make align suppress number for \\* lines
% define galign to use subequation labels
\makeatletter
\let\oldalign\align
\let\endoldalign\endalign

\newcommand*\numberthis[1][]{\stepcounter{equation}\tag{\theequation}}

%\ifconf{}{
%	\renewenvironment{align}{%
%		\begingroup%
%		\let\oldhalign\halign
%		\def\halign{%
%			\let\oldbreak\\%
%			\def\nonnumberbreak{\nonumber\oldbreak*}%
%			\def\\{%
%				\@ifstar{\nonnumberbreak}{\oldbreak}%
%			}%
%			\oldhalign%
%		}
%		\let\oldlabel\label%
%		\oldalign%
%	}{%
%		\endoldalign%
%		\endgroup%
%	}
%}

\newenvironment{galign}[1][]{%
	\subequations%
	#1%
%	\def\theequation{\theparentequation--\alph{equation}}%
	\def\theequation{\theparentequation{\protect\footnotesize\hspace{.1em}.\arabic{equation}}}%
%	\def\theequation{\theparentequation\rlap{~\,--\,\alph{equation}}}%
	\align%
}{%
	\endalign%
	\endsubequations%
}

%http://tex.stackexchange.com/a/309558
\newcommand\splitaftercomma[1]{%
  \begingroup
  \begingroup\lccode`~=`, \lowercase{\endgroup
    \edef~{\mathchar\the\mathcode`, \penalty0 \noexpand\hspace{0pt plus .25em}}%
  }\mathcode`,="8000 #1%
  \endgroup
}


\newcommand\tagref[2][\width]{%
	\tag*{\makebox[#1][r]{\wref{#2} \scriptsize revisited}}%
}


\newcommand\separatedpar{%
	\medskip
	\plaincenter{%
		$*$\hspace{3em}$*$\hspace{3em}$*$%
	}\par
	\medskip
	\noindent
}


% Notation list
\def\mydots{\xleaders\hbox to.5em{\hfill.\hfill}\hfill}


\newlength\tmpLenNotations
\newenvironment{notations}[1][10em]{%
	\small
	\newcommand\notationentry[1]{%
		\settowidth\tmpLenNotations{##1}%
		\ifthenelse{\lengthtest{\tmpLenNotations > \labelwidth}}{%
			\parbox[b]{\labelwidth}{%
				\makebox[0pt][l]{##1}\\%
			}%
		}{%
			\mbox{##1}%
		}%
		\mydots\relax%
	}%
	\begin{list}{}{%
		\setlength\labelsep{0em}%
		\setlength\labelwidth{#1}%
		\setlength\leftmargin{\labelwidth+\labelsep+1em}%
		\renewcommand\makelabel{\notationentry}%
	}
	\ifdraft{%
		\newcommand\notation[1]{%
			\item[{##1}] \marginpar{%
				\adjustbox{scale={.55}{1},outer}{%
					\color{brown!80}%
					\scriptsize$\triangleright$\;\tiny\texttt{\detokenize{##1}}%
				}%
			}%
		}%
	}{%
		\newcommand\notation[1]{\item[{##1}]}%
	}%
	\raggedright
}{%
	\end{list}
}
\newcommand*\phdthesis{\mbox{Ph.\hspace{.2ex}D.} thesis\xspace}


%%%%% Allow page breaks in display math environments 
%%%%% With this, display environments can be broken as paragraphs.
%%%%% The 1 means that such breaks should be considered not nice, but acceptable.
\allowdisplaybreaks[3]

%\ifconf{
	\let\oldparagraph\paragraph
	\renewcommand\paragraph[1]{%
		\oldparagraph*{#1}
	}
%}{
%	\let\oldparagraph\paragraph
%	\renewcommand\paragraph[1]{%
%		\oldparagraph{#1.}
%	}
%}

% !BIB program = bibtex
\bibliographystyle{plainurl}

\let\oldthebibliography\thebibliography
\renewcommand\thebibliography[1]{%
	\oldthebibliography{#1}%
	\pdfbookmark[1]{References}{}%
%	\sectionmark{Bibliography}%
%	\markright{References}
}


%\def\myacknowledgements{}
%\ifarxiv{
%	\newcommand\acknowledgements[1]{\def\myacknowledgements{\paragraph{Acknowledgements}#1}}
%}{}





\ifdraft{%
	% Show overfull boxes (without activating draft mode)
	\overfullrule=6mm
	
	%%%% Hacks to show labels, ref and cite keys
	\usepackage[color,notref,notcite]{showkeys}
	\definecolor{refkey}{gray}{.99}
	\colorlet{labelkey}{green!60!black!60}
	\renewcommand{\showkeyslabelformat}[1]{%
	  \adjustbox{scale={.6}{.9}}{\scriptsize{\texttt{#1}}}%
	}
	\usepackage[inline,nolabel]{showlabels}
	\renewcommand{\showlabelsetlabel}[1]{%
	  \adjustbox{scale={.6}{.9}}{\textcolor{blue!50!black!45}{\scriptsize{\texttt{#1}}}}%
	}
	\renewcommand\showlabelrefline{%
		\color{blue!55!black!35}\hrule width 0pt height 1.5ex depth 0pt%
	}
	\showlabels{cite}
	\showlabels{citealt}
	\showlabels{citealp}
	\showlabels{citet}
	\showlabels{Citet}
	\showlabels{citep}
	\showlabels{citeauthor}
	\showlabels{Citeauthor}
	\showlabels{citefullauthor}
	\showlabels{citeyear}
	\showlabels{citeyearpar}
	\showlabels{wref}
	\showlabels{wpref}
	\showlabels{wtpref}
	\showlabels{wildref}
	\showlabels{wildpageref}
	\showlabels{wildtpageref}
}{}

\ifdraft{}{%
	\usepackage{microtype}
}

\let\epsilon\varepsilon


\newsavebox\tmpbox

\raggedbottom

\makeatother

